$O(\sqrt{T})$ Static Regret and Instance Dependent Constraint Violation for Constrained Online Convex Optimization

The constrained version of the standard online convex optimization (OCO) framework, called COCO is considered, where on every round, a convex cost function and a convex constraint function are revealed to the learner after it chooses the action for that round. The objective is to simultaneously minimize the static regret and cumulative constraint violation (CCV). An algorithm is proposed that guarantees a static regret of $O(\sqrt{T})$ and a CCV of $\min\{\cV, O(\sqrt{T}\log T) \}$, where $\cV$ depends on the distance between the consecutively revealed constraint sets, the shape of constraint sets, dimension of action space and the diameter of the action space. For special cases of constraint sets, $\cV=O(1)$. Compared to the state of the art results, static regret of $O(\sqrt{T})$ and CCV of $O(\sqrt{T}\log T)$, that were universal, the new result on CCV is instance dependent, which is derived by exploiting the geometric properties of the constraint sets.

==> AppUnsync.tex <==
\section{Proof of Theorem \ref{lem:movementcost}}
\begin{proof}
We need the following preliminaries.

 \begin{definition}\label{defn:avgwidth}
Let $K$ be a non-empty convex bounded set in $\bbR^d$. Let $u$ be a unit vector, and $\ell_u$ a line through the origin parallel to $u$. 
Let $K_u$ be the orthogonal projection of $K$ onto $\ell_u$, with length $|K_u|$. The mean width of $K$ is defined as 
\begin{equation}\label{eq:projlength}
W(K) = \frac{1}{V_d} \int_{\bbS_1^d} |K_u| du,
\end{equation}
where $\bbS_1^d$ is the unit sphere in $d$ dimensions and $V_d$ its $(d-1)$-dimensional Lebesgue measure.
\end{definition}


The following is immediate. 
\begin{equation}\label{eq:WBound1}
0\le W(K) \le \text{diameter}(K).
\end{equation}

\begin{lemma}\label{lem:width2D}\cite{eggleston1966convexity}
For $d=2$, $$W(K)=\frac{\text{Perimeter}(K)}{\pi}.$$
\end{lemma}
Lemma \ref{lem:width2D} implies that $W(K) \ne W(K_1) + W(K_2)$ even if $K_1\cup K_2=K$ and $K_1\cap K_2=\phi$.




Recall from \eqref{defn:genconvxmovement} that $x_t\in  \partial S_{t-1}$ and $p_t$ is the projection of $x_t$ onto $S_{t}$, and $m_t$ is the mid-point of $x_t$ and $p_t$, i.e. $m_t = \frac{x_t+p_t}{2}$. Moreover, the convex sets $S_t$'s are nested, i.e., $S_1\supseteq S_2 \supseteq \dots \supseteq S_T$.
To prove Theorem \ref{lem:movementcost} we will bound the rate at which $W(S_t)$ (Definition \ref{defn:avgwidth}) decreases as a function of the length $||x_t-p_t||$. 

From Definition \ref{defn:anglewidth}, recall that $\cC_t$ is the convex hull of $m_t\cup S_{t}$. We also need to define $\cC_t^-$ as the convex hull of $x_t\cup S_{t}$. Since 
$S_t \subseteq \cC_t$ and $\cC_t^- \subseteq S_{t-1}$, we have \begin{equation}\label{eq:widthlb}
W(S_{t}) - W(S_{t-1}) \le W(\cC_t) - W(\cC_t^-).
\end{equation} 
\begin{definition}\label{}
$\Delta_t = W(\cC_t) - W(\cC_t^-)$.
\end{definition}
%and derive a bound on $\Delta_t$.



The main ingredient of the proof is the following Lemma that bounds  $\Delta_t$ whose proof is provided after completing the proof of Theorem \ref{lem:movementcost}.
\begin{lemma}\label{lem:derivative} $$\Delta_t  \le -V_{d-1}\frac{||x_t-p_t||}{2V_d(d-1)}  (c_t^\star)^{d},$$
where $c_t^\star$ has been defined in Definition \ref{defn:anglewidth}.
\end{lemma}


Recalling that $c^\star = \min_t  c^\star_t$ from Definition \ref{defn:anglewidth}, and  combining  Lemma \ref{lem:derivative} with \eqref{eq:WBound1} and \eqref{eq:widthlb}, we get that 
$$\sum_{t=1}^T ||x_t-p_t|| \le \frac{2V_d(d-1)}{V_{d-1}} \left(\frac{1}{c^\star}\right)^{d}\text{diameter}(S_1),$$
since $S_1\supseteq S_2 \supseteq \dots \supseteq S_T$. Recalling that $\text{diameter}(S_1)\le D$, Theorem \ref{lem:movementcost} follows.
\end{proof}
%Note that $b_t$ being a projection of $a_t$ onto 
%$S_{t}$, 

\begin{proof}[Proof of Lemma \ref{lem:derivative}]
% \begin{figure}[]
%  \begin{center}
%%\begin{tikzpicture}
%\begin{tikzpicture}[scale=1.5, dot/.style={circle,inner sep=1pt,fill,label={#1},name=#1},
%  extended line/.style={shorten >=-#1,shorten <=-#1},
%  extended line/.default=1cm]
%% Define coordinates
%\coordinate (w_t) at (0,0);
%\coordinate (z_t) at (0,-.5);
%\coordinate (x_t) at (-1,-1);
%\coordinate (y_t) at (1,0);
%\coordinate (C_top) at (1,2.15);
%\coordinate (C_bottom) at (3.55,-0.55);
%
%
%% Draw object (shaded region)
%%\draw[thick, gray, fill=pink!50] (C_top) to[out=-.5,in=-15] (C_bottom) -- cycle;
%
%
%
%
%
%% Draw projected image (S_t+1)
%\draw[thick, cyan, fill=cyan!50,opacity=0.75] (1,0) -- (1.5,1.5) -- (3,1) -- (3.2,0.15)  -- cycle;
%\draw[thick, blue!10, fill=blue!10,opacity=0.5] (z_t) --(1.5,1.495) --  (y_t)   -- cycle;
%\draw[thick, blue!10, fill=blue!10,opacity=0.5] (z_t) --  (y_t)  -- (3.2,0.15) -- cycle;
%
%\filldraw[blue] (y_t) circle (2pt) node[below right] {$b_t$};
%\filldraw[black] (z_t) circle (2pt) node[below right] {$m_t$};
%% Draw camera and viewing ray
%\draw[thick,->] (x_t) -- (y_t);
%\draw[dashed,->] (.65,0) -- (z_t) -- (-0.65,-1)  node[below right] {$w_t$};
%\draw[dashed,->] (.65,0) -- (z_t) -- (-0.65,-1)  node[below right] {$w_t$};;
%%\draw[dashed,->] (.65,0) -- (x_t) -- (-0.65,-1)  node[below right] {$w_t$};;
%
%\coordinate (u_1) at (0,.5);
%\coordinate (u_2) at (0,-2);
%
%\draw [ dashed, <-] (-1,.5) -- (x_t) -- (-1,-2) node[above left] {$H_u'$};
%\draw [ dashed, <-] (u_1) -- (z_t) -- (u_2) node[above left] {$H_u$};
%\draw [ dashed, ->] (1.3,-.7) -- (z_t) -- (-2.8,.2) node[above left] {$u$};
%
%%\draw [extended line, ->] ($(u_1)!(z_t)!(u_2)$) -- (-.5,-0.05) node[above left ] {$u$};
%
%%\draw [extended line,<-] ($(-0.25,.5)!(z_t)!(.25,-2)$) node[above left] {$u$};
%
%%\tkzDefLine[orthogonal=through (z_t)](x_t,y_t);
%
%
%%\filldraw[black] (w_t) circle (2pt) node[above left] {$w_t$};
%\filldraw[black] (x_t) circle (2pt) node[below left] {$a_t$};
%
%\draw[thick, gray, fill=pink!50,opacity=0.6] (C_top) to[out=.5,in=25] (C_bottom) -- cycle;
%
%\draw[thick, gray, fill=gray!50,opacity=0.6] (C_bottom) to[out=-155,in=-165] (C_top) -- cycle;
%\node at (2.25,0.75) {$S_{t}$};
%
%% Draw lines connecting camera to object and projected image
%\draw[dotted] (z_t) -- (1.5,1.5);
%\draw[dotted] (z_t) -- (3.2,0.15);
%%\draw[dotted] (w_t) -- (3,1);
%%\draw[dotted] (w_t) -- (2.5,0.5);
%%\draw[dotted] (w_t) -- (1.5,0.5);
%\draw[dotted] (z_t) -- (C_top);
%\draw[dotted] (z_t) -- (C_bottom);
%
%% Add labels for object and camera
%\node[above right] at (C_top) {$C_{w_t}(c_t)$};
%\end{tikzpicture}
%\caption{Figure representing the cone $C_{w_t}(c_t)$ that contains the convex hull of $m_t$ and $S_{t}$ with respect to the unit vector $w_t$. $u$ is a unit vector perpendicular to $H_u$ an hyperplane that is a supporting hyperplane $C_t$ at $m_t$ such that $\cC_t \cap H_u = \{m_t\}$ and 
%$u^T (a_t-m_t)\ge 0$ }
%\label{fig:anglewidth}
%\end{center}
%\end{figure}

\begin{figure*}
\begin{center}
\includegraphics[width=10cm,keepaspectratio,angle=0]{FigConeDefHyperplane.png}
\caption{Figure representing the cone $C_{w_t}(c_t)$ that contains the convex hull of $m_t$ and $S_{t}$ with respect to the unit vector $w_t$. $u$ is a unit vector perpendicular to $H_u$ an hyperplane that is a supporting hyperplane $C_t$ at $m_t$ such that $\cC_t \cap H_u = \{m_t\}$ and 
$u^T (x_t-m_t)\ge 0$ }
\label{fig:anglewidth}
\end{center}
\end{figure*}



Let $H_u$ be the hyperplane perpendicular to vector $u$.
 Let $\cU_0$ be the set of unit vectors $u$ such that hyperplanes $H_u$ are supporting hyperplanes to $\cC_t$ at point $m_t$ such that $\cC_t \cap H_u = \{m_t\}$ and 
$u^T (x_t-m_t)\ge 0$.  See Fig. \ref{fig:anglewidth} for reference.

 Since $p_t$ is a projection of $x_t$ onto $S_{t}$, and $m_t$ is the mid-point of $x_t,p_t$, for $u\in \cU_0$, the hyperplane $H_u'$ containing $x_t$ and parallel to $H_u$ is a supporting hyperplane for $\cC_t^-$.  


Thus, using the definition of $K_u$ from \eqref{eq:projlength},
\begin{equation}\label{eq:dummy1}
\Delta_t  \le \frac{1}{V_d} \int_{\cU_0} (|\cC_{t,u}| - |\cC_{t,u}^-|) du= -\frac{||x_t-p_t||}{2V_d} \int_{\cU_0} u^T 
\frac{(x_t-m_t)}{||x_t-m_t||}  \ du,
\end{equation}
since $||x_t-m_t|| = ||x_t-p_t||/2$.

Recall the definition of $C_{w_t^\star}(c_t^\star)$ from Definition \ref{defn:anglewidth} which implies that the convex hull of $m_t$ and $S_{t}$, $\cC_t$ is contained in $C_{w_t^\star}(c_t^\star)$.
Next, we consider $\cU_1$ the set of unit vectors $u$ such that hyperplanes $H_u$ are supporting hyperplanes to $C_{w_t^\star}(c_t^\star)$ at point $m_t$ 
such that $u^T (x_t-m_t)\ge 0$. 
By definition $\cC_t\subseteq C_{w_t^\star}(c_t^\star)$, it follows that 
$\cU_1\subset \cU_0$.

Thus, from \eqref{eq:dummy1}
 \begin{equation}\label{eq:dummy2}
\Delta_t  \le -\frac{||x_t-p_t||}{2V_d} \int_{\cU_1} u^T. \frac{(x_t-m_t)}{||x_t-m_t||} du
\end{equation}

Recalling the definition of $w_t^\star$ (Definition \ref{defn:anglewidth}), 
vector $u\in \cU_1$ can be written as 
$$ u = \lambda u_{\perp} + \sqrt{1-\lambda^2} w_t^\star,$$
where $u_{\perp}^T w_t^\star=0$, $|u_{\perp}|=1$ and since $u\in \cU_1$
$$0 \le \lambda=\sqrt{1-(u^Tw_t^\star)} = u^Tu_{\perp}\le c_t^\star.$$

Let $\cS_{\perp} = \{u_\perp: |u_\perp|=1 , u_\perp^T w_t^\star=0\}$. Let $du_{\perp}$ be the 
$(n-2)$-dimensional Lebesgue measure of $\cS_{\perp}$. 

It is easy to verify that 
$du = \lambda^{d-2}(1-\lambda^2)^{-1/2} d\lambda du_{\perp}$ and hence from \eqref{eq:dummy2}

\begin{equation}\label{eq:dummy3}
\Delta_t  \le -\frac{||x_t-p_t||}{V_d} \int_{0}^{c_t^\star}  \lambda^{d-2}(1-\lambda^2)^{-1/2} d\lambda \int_{\cS_{\perp}} (\lambda u_{\perp} + \sqrt{1-\lambda^2} w_t^\star)^T \frac{(x_t-m_t)}{||x_t-m_t||}  du_{\perp}.
\end{equation}
 
 Note that $\int_{du_{\perp}} u_{\perp} du_{\perp}=0$. Thus,
 \begin{align}\nn \label{}
\Delta_t  & = -\frac{||x_t-p_t||}{2V_d} \frac{(w_t^\star)^T(x_t-m_t)}{||x_t-m_t||}  \int_{0}^{c_t^\star}  \lambda^{d-2}(1-\lambda^2)^{-1/2}   \sqrt{1-\lambda^2}\ d\lambda   \int_{\cS_{\perp}} du_{\perp},\\ 
\nn
& \stackrel{(a)}\le -V_{d-1} \frac{||x_t-p_t||}{2V_d}  \frac{ (w_t^\star)^T(x_t-m_t)}{||x_t-m_t||}  \int_{0}^{c_t^\star} \lambda^{d-2}\ d\lambda, \\ \nn
& \stackrel{(b)}\le  -V_{d-1}\frac{||x_t-p_t||}{2V_d(d-1)} c_t^\star (c_t^\star)^{d-1},\\ 
& = -V_{d-1}\frac{||x_t-p_t||}{2V_d(d-1)}  (c_t^\star)^{d},
\end{align}
where $(a)$ follows since  $\int_{\cS_{\perp}} du_{\perp} = V_{d-1}$ by definition, $(b)$ follows since $ \frac{(w_t^\star)^T(x_t-m_t)}{||x_t-m_t||} \ge c_t^\star$ from Definition \ref{defn:anglewidth}.

%Clearly, $W(S_{t} - W(S_t) \ge \Delta_t$. 
%We will bound $\Delta_t $ to get a bound on the movement cost $M$ \eqref{eq:totalDistance}
 \end{proof}
 Note that the proof is conceptually similar to the proof of Theorem \ref{thm:manselli} in \cite{Manselli}, 
 and has been adapted to fit the considered problem.
